A generalized Hopfield model to store and retrieve mismatched memory patterns

We study a class of Hopfield models where the memories are represented by a mixture of Gaussian and binary variables and the neurons are Ising spins. We study the properties of this family of models as the relative weight of the two kinds of variables in the patterns varies. We quantitatively determine how the retrieval phase squeezes towards zero as the memory patterns contain a larger fraction of mismatched variables. As the memory is purely Gaussian retrieval is lost for any positive storage capacity. It is shown that this comes about because of the spherical symmetry of the free energy in the Gaussian case. Introducing two different memory pattern overlaps between spin configurations and each contribution to the pattern from the two kinds of variables one can observe that the Gaussian parts of the patterns act as a noise, making retrieval more difficult. The basins of attraction of the states, the accuracy of the retrieval and the storage capacity are studied by means of Monte Carlo numerical simulations. We uncover that even in the limit where the network capacity shrinks to zero, the (few) retrieval states maintain a large basin of attraction and large overlaps with the mismatched patterns. So the network can be used for retrieval, but with a very small capacity.

==> MyBibTex.tex <==
\begin{thebibliography}{99}

\bibitem{Agliari2:article}
E. Agliari et al. "Replica symmetry breaking in neural networks: a few steps toward rigorous results." Journal of Physics A: Mathematical and Theoretical 53.41 (2020): 415005.


\bibitem{Agliari1:article}
E. Agliari, F. Alemanno, A. Barra and A. Fachechi,
arXiv:1812.09077 (2018).

\bibitem{ImmuneNetworks2013}
E.~Agliari, A.~Annibale, A.~Barra, A.C.C.~Coolen and D.~Tantari, Journal of Physics A: Mathematical and Theoretical 46 (2013) 335101.

\bibitem{Agliari:article}
E. Agliari, A. Barra, C. Longo, D. Tantari, J. Stat. Phys. 168 (2017) 1085.

\bibitem{Aguirre:article}
F. Aguirre-Lopez, M. Pastore and S. Franz,
arXiv:2204.03577 (2022).


\bibitem{Amit2:article}
D. J. Amit, H. Gutfreund and H. Sompolinski, Phys. Rev. A 32  (1985) 1007.

\bibitem{Amit:article}
D. J. Amit, H. Gutfreund and H. Sompolinski, Annals of Physics 173 (1987) 30.

\bibitem{Amit:book}
D. J. Amit, "Modeling brain function: the world of attractor neural networks" (1989). 

\bibitem{Aquaro:article}
M, Aquaro, F. Alemanno, I. Kanter, F. Durante, E. Agliari and A. Barra, 
arXiv:2204.07954v1 (2022).

\bibitem{Barra:article}
A. Barra, G. Genovese, P. Sollich and D. Tantari,
Phys. Rev. E 96 (2017) 042156.

\bibitem{Barra1:article}
A. Barra, G. Genovese, P. Sollich and D. Tantari,
Phys. Rev. E 97, (2018) 022310.

\bibitem{Benedetti:article}
M. Benedetti, E. Ventura, E. Marinari, G. Ruocco and F. Zamponi, arXiv:2201.00032 (2022).

\bibitem{Bovier:article}
A. Bovier, A. C. D. van Enter and B. Niederhauser, J. Stat. Phys. 95 (1999) 181.
 
\bibitem{Crisanti:article}	
A. Crisanti, D.J. Amit and H. Gutfreund, Europhys. Lett. 2 (1986) 337.

\bibitem{Dominicis:article}
C. De Dominicis, M. Gabay and H. Orland, J. Physique Lett. 42 (1981) L523.

\bibitem{Fachechi:article}
A. Fachechi, E. Agliari and A. Barra,
arXiv:1810.12217 (2018).

\bibitem{Hebb:article}
D.O. Hebb, "The organization of Behaviour", Wiley, New York, 1949.

\bibitem{RBM2:article}
G. E. Hinton, Neural Comp. 14, 1771 (2002).

\bibitem{capacity1:article}
H. Homer, D. Bormann, M. Frick, H. Kinzelbach and A. Schmidt, Z. Phys. B 76 (1989) 381.

\bibitem {Hopfield:article}
J. J. Hopfield, Proc. Natl. Acad. Sci. U.S.A. 79 (1982) 2554; 81 (1984) 3088; J. J. Hopfield, D. I. Feinstein and R. G. Palmer, Nature 304 (1983) 158.

\bibitem{Winzel:article}
W. Kinzel, Phys. Rev. B 33 (1985) 5086.

\bibitem{SK:article}
S. Kirkpatrick, D. Sherrington. Phys. Rev. B 17 (1978) 4384.
 
\bibitem{capacity2:article}
G.A. Kohring, J. Stat. Phys. 59 (1990) 1077.

\bibitem{Ruocco:article}
M. Leonetti, E. Hormann, L. Leuzzi, G. Parisi and G. Ruocco, PNAS (2021) 118.
 
\bibitem{Little:article}
 W.A. Little, Math. Biosci. 19 (1974) 101.
 
\bibitem{LittleShaw:article}
W.A. Little and G.L. Shaw, Behav. Biol. 14 (1975) 115.


\bibitem{Mattis:article}
D.C. Mattis, Physics Letters A 56 (1976) 421.
  
\bibitem{MPV:book}
M. Mezard, G. Parisi, M. A Virasoro, "Spin Glass Theory and Beyond", World Scientific (1987).

\bibitem{Ramsauer:article}
H. Ramsauer, B. Sch\"afl, J. Lehner, P. Seidl, M. Widrich, T. Adler, L. Gruber, M. Holzleitner, M. Pavlovi\'c, G. K. Sandve, V. Greiff, D. Kreil, M. Kopp, G. Klambauer, J. Brandstetter, S. Hochreiter	arXiv:2008.02217 (2020).

\bibitem{RBM1:article}
P. Smolensky, Information Processing in Dynamical Systems
(MIT Press, Cambridge, MA, 1986).

\bibitem{Steffan:article}
H. Steffan, PhD thesis, Heidelberg, unpublished (1993); 

\bibitem{Steffan1:article}
H. Steffan and R. K{\"u}hn, "Replica symmetry breaking in at- tractor neural network models." Zeitschrift f{\"u}r Physik B Condensed Matter 95.2 (1994): 249-260.

\bibitem{Stiefvater:article}
T. Stiefvater, K. R. Miiller, R. Kuhn, Physica A 232 (1996) 61.

\bibitem{capacity3:article}
K. Tokita, J. Phys. A 27 (1994) 4413. 

\bibitem{Enter:article}
A. C. D. Van Enter and H. G. Schaap, J. Phys. A: Math. Gen. 35 (2002) 2581.
\end{thebibliography}
